Discovery of the Closest Ultrastripped Supernova: SN 2021agco in UGC 3855

We present the discovery and studies of the helium-rich, fast-evolving supernova (SN) 2021agco at a distance of $\sim$ 40 Mpc. Its early-time flux is found to rise from half peak to the peak of $-16.06\pm0.42$ mag in the $r$ band within $2.4^{+1.5}_{-1.0}$ days, and the post-peak light curves also decline at a much faster pace relative to normal stripped-envelope SNe of Type Ib/Ic. The early-time spectrum of SN~2021agco ($t \approx 1.0$ days after the peak) is characterized by a featureless blue continuum superimposed with a weak emission line of ionized C III, and the subsequent spectra show prominent He I lines. Both the photometric and spectroscopic evolution shows close resemblances to SN 2019dge, which is believed to have an extremely stripped progenitor. We reproduce the multicolor light curves of SN 2021agco with a model combining shock-cooling emission with \Ni decay. The best-fit results give an ejecta mass of $\approx 0.3$~M$_\odot$ and a synthesized nickel mass of $\approx 2.2\times10^{-2}$~M$_\odot$. The progenitor is estimated to have an envelope radius $R_{\rm env} \approx 80$~R$_\odot$ and a mass $M_{\rm env} \approx 0.10$~M$_\odot$. All these suggest that SN~2021agco can be categorized as an ultrastripped SN~Ib, representing the closest object of this rare subtype. This SN is found to explode in the disk of an Sab-type galaxy with an age of $\sim 10.0$~Gyr and low star-forming activity. Compared to normal SNe Ib/c, the host galaxies of SN 2021agco and other ultrastripped SNe tend to have relatively lower metallicity, which complicates the properties of their progenitor populations.

==> FitResultTable.tex <==
\begin{table}
\caption{Parameters Determined from MCMC Fit to the Observed Multicolor Light Curves of SN 2021agco}
    \centering
    \begin{tabular}{ccc}
        \hline
        \hline
        ~ &  \Ni Decay & Shock Cooling + \Ni Decay\\
        $\theta$               & Value & Value  \\
        \hline
        log $M_{\rm Ni}$  & $-1.60_{-0.01}^{+0.01}$   &  $-1.85_{-0.01}^{+0.01}$\\
        $\tau_{\rm diff}$          & $1.51_{-0.00}^{+0.01}$ d  &  $4.82_{-0.27}^{+0.29}$ d\\
        $\tau_{\gamma}$        & $10.71_{-0.21}^{+0.21}$ d &  $17.67_{-0.60}^{+0.60}$ d\\
        $E_{\rm ext}$     & -                         & $3.13_{-0.34}^{+0.40}\times 10^{49}~erg$ \\
        $R_{\rm ext}$     & -                         & $117.07_{-12.34}^{+14.03}$ \rsun\\
        $M_{\rm ext}$     & -                         & $0.08_{-0.01}^{+0.01}$ \msun\\
        \hline
    \end{tabular}
%    \caption{Parameters Determined from MCMC Fit to the Observed Multicolor Light Curves of SN 2021agco}
    \label{tab: MCMCresult}
\end{table}

==> figures/Exp_param_USSNe.tex <==
\begin{table}
    \label{tab: Exp_param_USSNe}
    \caption{The explosion parameters of suggested ultra-striped envelope supernovae}
    \begin{threeparttable}
        \centering
        \begin{tabular}{cc}
            \hline
            \hline
            Transient & Redshift & Host Galaxy & Second Peak & Decay Rate (g-band) & Ejecta Mass            & Nickel Mass                    & Envelope Radius    & Envelope Mass 
            Name      &          & Type        & Magnitude   & (mag day^{-1})      & $M_{ej}$ ($M_{\odot}$) & $M_{Ni}$ ($10^{-2} M_{\odot}$) & $R_{ext}$ ($10^{13}$ cm) & $M_{ext}$ ($10^{-2} M_{\odot}$)
            \hline
            % $E_k=3.79\times10^{49}_{-0.33}^{+0.36}~erg$, 
            % $M_{ejecta}=0.19_{-0.02}^{+0.02}$ \msun 
            % $M_{Ni}=0.0012_{-0.01}^{+0.01}$ \msun. 
            % $R_{env}=113.2_{-9.8}^{+11.7}$ \rsun, 
            % $M_{env}=0.11_{-0.01}^{+0.01}$ \msun and the 
            % $E_{env}=3.68\times10^{50}_{-0.33}^{+0.36}~erg$.
            SN2021agco& 0.01056& Spiral  &       $\pm$      &                      & 0.19_{-0.02}^{+0.02} & 1.9_{-2}^{+2}         & 0.78^{+0.09}_{-0.06}
            AT2019wxt & 0.036  & Compact & -16.6 $\pm$ 0.41 & 0.20^{+0.12}_{-0.11} & 2.73^{+0.33}_{-0.18} & 35.8^{+4.06}_{-3.68}  & 3.55^{+0.12}_{-0.11}
            SN2019dge & 0.021  & Compact & -15.5 $\pm$ 0.13 & 0.38^{+0.02}_{-0.02} & 1.57^{+0.04}_{-0.03} & 1.19^{+0.06}_{-0.05}  & 9.71^{+0.28}_{-0.27}
            iPTF14gqr & 0.063  & Spiral  & -17.5 $\pm$ 0.21 & 0.24^{+0.02}_{-0.02} & 8.14^{+0.14}_{-0.15} & 6.09^{+8.73}_{-3.18}  & 2.59^{+0.46}_{-0.34}
            iPTF16hgs & 0.017  & Spiral  & -15.1 $\pm$ 0.17 & 1.68^{+0.28}_{-0.25} & 2.51^{+0.20}_{-0.22} & 2.45^{+14.08}_{-1.80} & 9.27^{+3.40}_{-2.48}
            \hline
        \end{tabular}
        \caption{The summary properties of the suggested ultra-stripped SNe, including the redshift and type of the host galaxy, light curve properties, i.e., the decay rate anf peak luminosity of the light curves, and explosion parameters inferred from the light curve fitting, i.g., ejecta mass $M_{ej}$, nickel mass $M_{Ni}$, envelope radius $R_{ext}$ envelope mass $M_{ext}$. Most information and parameters refer from the \cite{AT2019wxt_2022arxiv,} and \cite{SN2019dge_2020ApJ}}
    \end{threeparttable}
\end{table}

